UniLCD: Unified Local-Cloud Decision-Making via Reinforcement Learning

Embodied vision-based real-world systems, such as mobile robots, require a careful balance between energy consumption, compute latency, and safety constraints to optimize operation across dynamic tasks and contexts. As local computation tends to be restricted, offloading the computation, ie, to a remote server, can save local resources while providing access to high-quality predictions from powerful and large models. However, the resulting communication and latency overhead has led to limited usability of cloud models in dynamic, safety-critical, real-time settings. To effectively address this trade-off, we introduce UniLCD, a novel hybrid inference framework for enabling flexible local-cloud collaboration. By efficiently optimizing a flexible routing module via reinforcement learning and a suitable multi-task objective, UniLCD is specifically designed to support the multiple constraints of safety-critical end-to-end mobile systems. We validate the proposed approach using a challenging, crowded navigation task requiring frequent and timely switching between local and cloud operations. UniLCD demonstrates improved overall performance and efficiency, by over 35% compared to state-of-the-art baselines based on various split computing and early exit strategies.

==> notes.tex <==

For supplementary - breakdown by type of scene. harsher scene? 

GPT: also on cloud. LLMs

Story is - local is more efficient. but can suffer performance/cost. Off loading can support smaller model inference locally. This is a nuanced point. 
RL is the main thing, as opposed to uncertainity heuristics, which more flexible. 
%Local is less. 
Local: larger and stronger models. 
use a little bit of cloud, get better performance. local only, performance is poor. 

only medium local
vs. 

Depend on the size of the image. 


Traina cloud model ,first few layers. 

Badnit. 
Imitation learning, vs. RL. 
Like Avis', state-independent. 

communication is fixed overhead, while models grow. 




\red{clarify siuational explicitly. Should we mention large foundation and language-based models, energy hungry more and more, massive compute that's difficult to run locally. }


"Harmonic Convergence: Unifying Local and Cloud Computation for Decision-Making Policies"
"Cloud-Local Symphony: Orchestrating Holistic Policies for Unified Decision-Making"
"Holistic Horizons: Blending Cloud and Local Wisdom in Decision Policies"
"United Skies and Grounds: Harmonizing Decision-Making through Cloud-Local Collaboration"
"Synchronized Strategies: Achieving Decision Harmony with Cloud-Local Integration"
"Seamless Fusion: Crafting Coherent Decision Policies in the Cloud-Local Continuum"
"Collaborative Cloudscapes: Building Decision Policies on Local-Cloud Harmony"
"EcoCloud Strategies: Fostering Ecosystemic Harmony in Cloud-Local Decision Making"
"Decision Weave: Interlacing Local Insights and Cloud Intelligence for Harmonized Policies"
"Harmony in Heterogeneity: Cloud-Local Collaborations for Enlightened Decision Policies"
"CloudRoots Confluence: Nurturing Decision Harmony in the Cloud-Local Nexus"
"Policy Polyphony: Harmonizing Local Voices and Cloud Visions for Decision Excellence"
"Unity in Diversity: Bridging Cloud and Local Dynamics for Holistic Decision Policies"
"Intertwined Intelligence: Forging Decision Harmony Between Cloud and Local Realms"
"Holistic Cloudscape: Crafting Integrated Decision Policies for Cloud-Local Ecosystems"
"Concordant Clouds: Aligning Local Realities with Cloud Capacities for Decision Synergy"
"Bridging Biomes: Harmonized Decision Policies for Cloud and Local Landscapes"
"Cloud-Local Consonance: Orchestrating Unified Policies for Informed Decision-Making"
"Harmonized Horizons: The Art of Cloud-Local Integration for Decision Policies"
"Collaborative Canopy: Weaving Together Cloud and Local Strands for Decision Harmony"



